Stochastic Adversarial Networks for Multi-Domain Text Classification

Adversarial training has been instrumental in advancing multi-domain text classification (MDTC). Traditionally, MDTC methods employ a shared-private paradigm, with a shared feature extractor for domain-invariant knowledge and individual private feature extractors for domain-specific knowledge. Despite achieving state-of-the-art results, these methods grapple with the escalating model parameters due to the continuous addition of new domains. To address this challenge, we introduce the Stochastic Adversarial Network (SAN), which innovatively models the parameters of the domain-specific feature extractor as a multivariate Gaussian distribution, as opposed to a traditional weight vector. This design allows for the generation of numerous domain-specific feature extractors without a substantial increase in model parameters, maintaining the model's size on par with that of a single domain-specific extractor. Furthermore, our approach integrates domain label smoothing and robust pseudo-label regularization to fortify the stability of adversarial training and to refine feature discriminability, respectively. The performance of our SAN, evaluated on two leading MDTC benchmarks, demonstrates its competitive edge against the current state-of-the-art methodologies. The code is available at https://github.com/wangxu0820/SAN.

==> tables/tb-parameters.tex <==
\begin{table}
\resizebox{1.0\columnwidth}{!}{
\begin{tabular}{l| c | c  }
  \toprule
  Task & Amazon & FDU-MTL \\
  \midrule
  \# Para. of $F_s$ & 5.57M & 20.20M  \\
  \# Para. of $\{F_d^i\}_{i=1}^M$ & 22.13M=4*5.57M & 322.65M=16*20.20M  \\
  \# Para. of $C$ & 0.04M & 0.04M \\
  \# Para. of $D$  & 0.02M & 0.02M \\
  \# Total Para.  & 27.76M & 342.91M \\
  \bottomrule
\end{tabular}}
\caption{The number of parameters of the shared feature extractor $F_s$, the domain-specific feature extractors $\{F_d^i\}_{i=1}^M$, the classifier $C$, and the domain discriminator $D$ in MAN \cite{chen2018multinomial} on different tasks. Obviously, the domain-specific feature extractor parameters take the majority part in both tasks. This means tackling more domains will drastically increase the model size.}
\label{tab222}
\end{table}
